Exploiting and Defending Against the Approximate Linearity of Apple's NeuralHash

Perceptual hashes map images with identical semantic content to the same $n$-bit hash value, while mapping semantically-different images to different hashes. These algorithms carry important applications in cybersecurity such as copyright infringement detection, content fingerprinting, and surveillance. Apple's NeuralHash is one such system that aims to detect the presence of illegal content on users' devices without compromising consumer privacy. We make the surprising discovery that NeuralHash is approximately linear, which inspires the development of novel black-box attacks that can (i) evade detection of "illegal" images, (ii) generate near-collisions, and (iii) leak information about hashed images, all without access to model parameters. These vulnerabilities pose serious threats to NeuralHash's security goals; to address them, we propose a simple fix using classical cryptographic standards.

==> proposal/goals.tex <==
\section{Project Goals} \label{sec:project-goals}

At a high level, our goals are to analyze the shortcomings of Apple's \nh (Section \ref{subsec:analysis}) and then propose improvements (Section \ref{subsec:improvement}).

\subsection{Analysis} \label{subsec:analysis}
Based on prior work done in literature and our knowledge of deep learning systems, we believe that two types of attacks will likely be effective against the current implementation of \nh. First, given public knowledge of the model, gradient based attacks can be used to turn innocuous images into those detected as CSAM, and vice versa. We will use standard deep learning tools for constructing adversarial attacks to do this \cite{goodfellow2014explaining}. 

However, particularly in the false negative case, we believe that it is likely unnecessary to have knowledge of the model. Given the lack of robustness of most DL systems, we are confident that even simple augmentations will inoculate images that should be classified as CSAM.

Note that to conduct these analyses we will not use images of CSAM, but will likely substitute out these images for those of another class (e.g. images of trees).

\subsubsection{Gradient-based Adversarial Attacks}
These attacks rely on knowing the model parameters of Apple's \nh system.

\noindent \textbf{i. False Positive Attack}: 
Given innocuous images, we will use knowledge of model parameters in Apple's\nh system and standard deep learning tools to construct images classified as CSAM while changing the image as little as possible \cite{goodfellow2014explaining}.

\noindent \textbf{ii. False Negative Attack}: 
Given images classified as CSAM, we will use knowledge of model parameters in Apple's\nh system and standard deep learning tools to construct images classified as innocuous while changing the image as little as possible \cite{goodfellow2014explaining}. 

\subsubsection{Black-box Adversarial Attacks}
These attacks rely on little to no knowledge of the inner workings of Apple's \nh system.

\noindent \textbf{i. Gaussian Noise}:
Given images classified as CSAM, we will identify the minimum level of Gaussian noise required to classify the image as innocuous. 

\noindent \textbf{i. Random Occlusions}:
Given images classified as CSAM, we will identify the minimum level of occlusions required to classify the image as innocuous.

\subsection{Proposed Improvements} \label{subsec:improvement} % <- someone think of a better verb
We have several ideas as to how we could improve the security of Apple's \nh system or potentially expand on top of it.

\begin{itemize}
    \item Extending Apple's system to applications with other data modalities such as videos, phone call audio, or text. These may be interesting to study from a national security vs data privacy perspective.  
    \item Rewrite the system to include a third party which serves as a maintainer of an up-to-date database of CSAM. This would allow the CSAM database that Apple checks against to be much more comprehensive as it does not need to be stored on each user's device. Rewriting the proposal to meet all the security guarantees would likely be a non-trivial challenge.  
    \item Improve \nh's perceptual algorithm to prevent adversarial attacks. One potential avenue for exploration would be to attempt to make the perceptual hash more difficult to cluster. Another approach would be to pull from the literature on making deep learning models more robust against these types of attacks \cite{madry2017towards}.
\end{itemize}

These ideas are certainly not final, but hopefully they provide a taste for the types of improvements we seek to make to \nh.

==> proposal/intro.tex <==
\section{Introduction}

In 2021, Apple unveiled \nh \cite{apple-nh}, a perceptual hashing system which aims to detect Child Sexual Abuse Material (CSAM) on images that are uploaded to iCloud.
The fundamental problem that \nh attempts to solve is one of great interest to the worldwide community: how can we efficiently surveil for various types of abuse \textit{without} compromising user privacy?
% A system that achieves this goal could find important applications in many areas not limited to the specific case of CSAM.

Unfortunately, \nh has been controversial since its release, due to concerns about its efficacy and about user privacy. These concerns have been made concrete, with recent work identifying problems with \nh's collision resistance, privacy guarantees, and false positive/negative rates under adversarial attacks \cite{breaking-nh-struppek, nh-repro-github, nh-collisions-github, nh-collisions-blog}.

% basically this is a fuzzy matcher, it's hard, ppl use deep elearning, but deeplearn ing is not to be trusted has lots of edge  cases needs analysis and imprvoement ?? 

Many issues with \nh arise from its usage of deep learning as the mechanism of hashing. Neural networks are employed because fuzzy image matching is extremely difficult even with rule-based or classical learning algorithms \cite{fuzzy-transforms, near-duplicate-im-detect}, but deep networks are also known to be sensitive to edge cases, susceptible to adversarial attacks, and prone to unexplainable behavior \cite{goodfellow2014explaining}. We believe that using our intuitions about deep learning will enable us to better investigate \nh's vulnerabilities and discover potential improvements to the system.
% As such, we will apply intuitions about deep learning to guide our investigation into the vulnerabilities of \nh. Specifically, we postulate that systems like \nh are vulnerable to adversarial attacks that have been shown to be effective on other deep learning systems . Neural networks often contain a multitude of edge cases that require further analysis and can provide insights into potential improvements to the system.

In this project proposal, we first describe the \nh system (Section \ref{sec:nh-background}), including its technical formulation and security goals. Then, we explain our goals for the project (Section \ref{sec:project-goals}): we will first focus on investigating the vulnerabilities of \nh, and then attempt to improve the system. Related work is covered in Section \ref{sec:related-work}.


==> proposal/nh-background.tex <==
\section{\nh Background} \label{sec:nh-background}

\subsection{Functional Specification} \label{subsec:nh-func-spec}

Apple's \nh CSAM Detection scheme, released with iOS 15, allows automatic detection of Child Sexual Abuse Material (CSAM) in photos that are uploaded to Apple's iCloud. This system depends on three major systems, which we will discuss here:
\begin{itemize}
    \item \nh
    \item Private Set Intersection
    \item Threshold Secret Sharing
\end{itemize}

\nh is a perceptual hashing system. In contrast with cryptographic hashing, \nh values for images preserve perceptual and semantic similarity. These hashes are generated in two steps. First, a neural network generates a floating-point vector ``descriptor'' that is a compressed representation of all of the key information in the image. Second, a technique known as Hyperplane Local Sensitivity Hashing \cite{lsh-wiki} converts these real-valued vectors into integer-valued vectors.

Private Set Intersection (PSI) \cite{apple-psi} is a communication protocol used between user's devices and Apple's servers. The PSI protocol is used to preserve user privacy by ensuring that Apple is unable to learn about users' images. It also creates a secure communication protocol for Apple to determine on the server-side if a user's photos match with existing CSAM images; this prevents adversarial attacks that would arise if users were able to easily determine which images would be flagged as CSAM and which would not. 

Finally, Threshold Secret Sharing prevents Apple from learning the encryption key specific to the user until the user has crossed a specific threshold for their number of matches with known CSAM content. After crossing this threshold, the user is able to decrypt information describing the specific CSAM content that the user's images matched with.

The neural network-based hashing algorithm will be at the core of our investigation. Deep networks are excellent fuzzy matchers, but they often suffer from unpredictable behavior, for example in the case of adversarial attacks. It is difficult to \textit{prove} their properties, which makes it all-the-more important that we empirically analyze their behaviors carefully, especially under adversarial conditions.

\subsection{Our Proposed Security Goals for \nh} \label{subsec:nh-security-goals}

Here, we define our idealized desiderata for \nh by examining all parties involved and describing a concrete security policy.

The parties involved with \nh are Apple with their servers and individual users with their devices and data. The primary objective of \nh is to protect the privacy of user data. Specifically, Apple should not be able to get any information about the semantic content of any images on a user's device. The only exception to this rule is that Apple should be able to query the user's device and get a boolean answer to the following question: are there at least 30 instances of CSAM on a user's device? Apple should be able to run this query at any time. 

Some more nuanced desired functionalities are as follows. In order to reduce the number of adversarial attacks to the \nh system, users should not know when they have a `match' with CSAM images in apple's database. Users may know when Apple runs a query on their device, but they should not be aware of the result of the query. This serves as a prevention measure for adversarial behavior. Finally, another desired property to reduce adversarial attacks is that even with public knowledge of all parts of the \nh system, it should be impossible (or at the very least, extremely computationally difficult) for an adversary to artificially construct images that result in false positives or false negatives to Apple's query.

This last desired functionality is one of the most difficult to guarantee, but is also one of the most important. Without this assumption, it may be possible for an adversary to hide CSAM on their device without Apple's knowledge. It may also be possible for an adversary to modify images on an innocent person's device in such a way that Apple detects CSAM.

Clearly, Apple is making a lot of promises with their \nh system. However, Apple uses deep learning, which traditionally suffers catastrophically from adversarial attacks, edge cases, and lack of robustness. This is why we conjecture that Apple's system does not match all the desired guarantees.

\subsection{Obtaining Authorization}
There are publicly released directions on how to access Apple's \nh models which can be found in releases of iOS 15 and above. For instance, see \href{https://github.com/AsuharietYgvar/AppleNeuralHash2ONNX}{this github repo}. Since we will be doing all testing on our local machines, we will not be exceeding our authorized access by working with these models.

\iffalse

- objectives/desired functionalities:
    - privacy to users (apple should not be able to see their images) 
    - users should not know when they have a "match" with CSAM images in apple's database (allows generation of adversarial images 
    - Apple shouldn’t be able to decrypt the CSAM until the encryption secret comes out 
- permissible actions 
    - Apple can query user devices at any time and should recieve a yes/no answer as to whether that user has CP on their device 
- unavailable actions 
    - apple should not be able to see 
    
- videos? phone calls? audio? 
- add a third party 
- do something to the perceptual hash to make it difficult to cluster 

Parties 
Permissible Actions 
Unavailable Actions 

Desired Objectives and Functionalities

Availability and Confidentiality Integrity
Detection vs Prevention

\fi

==> proposal/rel-work.tex <==
\section{Related Work} \label{sec:related-work}

\subsection{Non-Neural Fuzzy Image Matching Algorithms}
Fundamentally, \nh aims to be a cryptographically-secure fuzzy matching algorithm, matching user images with a large database while invariant under various kinds of transformations: blurring, cropping, rotation, stretching, shearing, etc. While \nh is driven by deep learning at its core, other approaches to this problem exist.
One approach \cite{fuzzy-transforms} applies F-Transforms to compute similarity measures between images, while another \cite{near-duplicate-im-detect} combines the minHash algorithm with TF-IDF weighting to generate similarity features.

\subsection{Failure Models of the \nh System}

Following \nh's public announcement, various attacks were proposed to defeat its security desiderata (Section \ref{subsec:nh-security-goals}). Broadly, researchers found issues with (i) collision resistance, (ii) computational distinguishability between different perceptual hashes, and (iii) adversarial attacks that artificially induced false positives and negatives.

\noindent \textbf{i. Collisions}: \cite{nh-collisions-blog, nh-collisions-github}
The system was designed to produce collisions on images that are the same, modulo perturbations due to JPEG encoding, resizing, or watermarks, while avoiding collisions for different images. However, naturally occurring collisions of different images have been found, where two images of different objects produce identical hashes even without artificial modification of the images themselves.

\noindent \textbf{ii. Computational Distinguishability}: \cite{breaking-nh-struppek}
A recent study showed that the cosine distance between hashes correlates with the strength of the semantic relationship between the original images. In other words, an adversary that gains access to the hashes of images can gain information about the original images; this could potentially be a serious security flaw.

\noindent \textbf{iii. Adversarial Attacks}: \cite{breaking-nh-struppek, goodfellow2014explaining}
Additionally, the weights of the \nh model have been extracted and made public, allowing for the artificial modification of images to produce desired hashes. Oftentimes, this artificial modification is not easily visually discernible. This has opened the door to attacks like transforming innocuous photos into those labelled as CSAM, or vice versa.

While these vulnerabilities have been publicly documented, we would like to explore them in greater depth, and also with the intent to (perhaps partially) resolve one or more of them.

==> report/nh-background.tex <==
\section{\nh Background} \label{sec:nh-background}

\subsection{Functional Specification} \label{subsec:nh-func-spec}

\begin{figure*}[h]
  \centering
  \includegraphics[keepaspectratio, width=1\textwidth]{figs/NeuralHash Diagram.png}
  \caption{NeuralHash Pipeline. Consists of a preprocessing step that transforms images into a consistent format. This is followed by an embedding network step and a Locality-Sensitive Hashing step. The output vector from the embedding network is compared with the hyperplanes in the hashing matrix to produce the output binary hash \cite{breaking-nh-struppek}.}
  \label{fig:NH-Diag}
\end{figure*}

Apple's \nh CSAM Detection scheme, released with iOS 15, allows automatic detection of Child Sexual Abuse Material (CSAM) in photos that are uploaded to Apple's iCloud. This system depends on three major systems, which we will discuss here:
\begin{itemize}
    \item \nh
    \item Private Set Intersection
    \item Threshold Secret Sharing
\end{itemize}

\nh is a perceptual hashing system. In contrast with cryptographic hashing, \nh values for images preserve perceptual and semantic similarity. These hashes are generated in two steps. First, a neural network generates a floating-point vector ``descriptor'' that is a compressed representation of all of the key information in the image. Second, a technique known as Hyperplane Local Sensitivity Hashing \cite{lsh-wiki} converts these real-valued vectors into integer-valued vectors.

Private Set Intersection (PSI) \cite{apple-psi} is a communication protocol used between user's devices and Apple's servers. The PSI protocol is used to preserve user privacy by ensuring that Apple is unable to learn about users' images. It also creates a secure communication protocol for Apple to determine on the server-side if a user's photos match with existing CSAM images; this prevents adversarial attacks that would arise if users were able to easily determine which images would be flagged as CSAM and which would not. 

Finally, Threshold Secret Sharing prevents Apple from learning the encryption key specific to the user until the user has crossed a specific threshold for their number of matches with known CSAM content. After crossing this threshold, the user is able to decrypt information describing the specific CSAM content that the user's images matched with.

The neural network-based hashing algorithm will be at the core of our investigation. Deep networks are excellent fuzzy matchers, but they often suffer from unpredictable behavior, for example in the case of adversarial attacks. It is difficult to \textit{prove} their properties, which makes it all-the-more important that we empirically analyze their behaviors carefully, especially under adversarial conditions.

\subsection{Idealized Security Goals for \nh} \label{subsec:nh-security-goals}

Here, we define our idealized desiderata for \nh by examining all parties involved and describing a concrete security policy.

The parties involved with \nh are Apple with their servers and individual users with their devices and data. The primary objective of \nh is to protect the privacy of user data. Specifically, Apple should not be able to get any information about the semantic content of any images on a user's device. The only exception to this rule is that Apple should be able to query the user's device and get a boolean answer to the following question: are there at least 30 instances of CSAM on a user's device? Apple should be able to run this query at any time. 

Some more nuanced desired functionalities are as follows. In order to reduce the number of adversarial attacks to the \nh system, users should not know when they have a `match' with CSAM images in apple's database. Users may know when Apple runs a query on their device, but they should not be aware of the result of the query. This serves as a prevention measure for adversarial behavior. Finally, another desired property to reduce adversarial attacks is that even with public knowledge of all parts of the \nh system, it should be impossible (or at the very least, extremely computationally difficult) for an adversary to artificially construct images that result in false positives or false negatives to Apple's query.

This last desired functionality is one of the most difficult to guarantee, but is also one of the most important. Without this assumption, it may be possible for an adversary to hide CSAM on their device without Apple's knowledge. It may also be possible for an adversary to modify images on an innocent person's device in such a way that Apple falsely detects CSAM.

Clearly, Apple is making a lot of promises with their \nh system. However, Apple uses deep learning, which traditionally suffers catastrophically from adversarial attacks, edge cases, and lack of robustness. This is why we conjecture that Apple's system does not match all the desired guarantees.

\subsection{Obtaining Authorization}
There are publicly released directions on how to access Apple's \nh models which can be found in releases of iOS 15 and above. For instance, see \href{https://github.com/AsuharietYgvar/AppleNeuralHash2ONNX}{this github repo}. Since we will be doing all testing on our local machines, we will not be exceeding our authorized access by working with these models.

\iffalse

- objectives/desired functionalities:
    - privacy to users (apple should not be able to see their images) 
    - users should not know when they have a "match" with CSAM images in apple's database (allows generation of adversarial images 
    - Apple shouldn’t be able to decrypt the CSAM until the encryption secret comes out 
- permissible actions 
    - Apple can query user devices at any time and should recieve a yes/no answer as to whether that user has CP on their device 
- unavailable actions 
    - apple should not be able to see 
    
- videos? phone calls? audio? 
- add a third party 
- do something to the perceptual hash to make it difficult to cluster 

Parties 
Permissible Actions 
Unavailable Actions 

Desired Objectives and Functionalities

Availability and Confidentiality Integrity
Detection vs Prevention

\fi

==> report/related_work.tex <==
\section{Related Work} \label{sec:related-work}

% \reminder{Stuff written here is from the proposal -- make sure that the main paper that we keep talking about in chat is cited and covered here. I already notice that the black box attacks they did (rotating, scewing the image) is not covered. Also they also tried to do image classification based on hash, that should also be written here}

\subsection{Non-Neural Fuzzy Image Matching Algorithms}
Fundamentally, \nh aims to be a cryptographically-secure fuzzy matching algorithm, matching user images with a large database while invariant under various kinds of transformations: blurring, cropping, rotation, stretching, shearing, etc. While \nh is driven by deep learning at its core, other approaches to this problem exist.
One approach \cite{fuzzy-transforms} applies F-Transforms to compute similarity measures between images, while another \cite{near-duplicate-im-detect} combines the minHash algorithm with TF-IDF weighting to generate similarity features.

\subsection{Failure Modes of the \nh System}

Following \nh's public announcement, various attacks were proposed to defeat its security desiderata (Section \ref{subsec:nh-security-goals}). Broadly, researchers found issues with (i) collision resistance, (ii) computational distinguishability between different perceptual hashes, (iii) adversarial attacks that artificially induced false positives and negatives, and (iv) non-robustness to basic image transformations.

\noindent \textbf{i. Collisions}: \cite{nh-collisions-blog, nh-collisions-github}
The system was designed to produce collisions on images that are the same, modulo perturbations due to JPEG encoding, resizing, or watermarks, while avoiding collisions for different images. However, naturally occurring collisions of different images have been found, where two images of different objects produce identical hashes even without artificial modification of the images themselves.

\noindent \textbf{ii. Computational Distinguishability}: \cite{breaking-nh-struppek}
A recent study showed that the cosine distance between hashes correlates with the strength of the semantic relationship between the original images. In other words, an adversary that gains access to the hashes of images can gain information about the original images; this could potentially be a serious security flaw.

\noindent \textbf{iii. Adversarial Attacks}: \cite{breaking-nh-struppek, goodfellow2014explaining}
Additionally, the weights of the \nh model have been extracted and made public, allowing for the artificial modification of images to produce desired hashes. Oftentimes, this artificial modification is not easily visually discernible. This has opened the door to attacks like transforming innocuous photos into those labelled as CSAM, or vice versa.

\noindent \textbf{iv. Black-Box Attacks}: \cite{breaking-nh-struppek}
In addition, certain black box attacks have been shown to be effective at changing the output of \nh, such as basic image transformations like translation, rotation, flipping, cropping, and brightness and contrast changes.

% While these vulnerabilities have been publicly documented, we would like to explore them in greater depth, and also with the intent to (perhaps partially) resolve one or more of them.

\subsection{Our Contributions}

In this paper, we improve on SOTA gradient-based attacks and provide stronger semantic guarantees than previous methods. We also propose an entirely novel class of powerful, black-box attacks using image interpolation. Finally, we propose and validate changes to the architecture as well as adversarial input detection to safeguard against some of the above attacks.

